Learning Heterogeneous Agent Cooperation via Multiagent League Training

Many multiagent systems in the real world include multiple types of agents with different abilities and functionality. Such heterogeneous multiagent systems have significant practical advantages. However, they also come with challenges compared with homogeneous systems for multiagent reinforcement learning, such as the non-stationary problem and the policy version iteration issue. This work proposes a general-purpose reinforcement learning algorithm named Heterogeneous League Training (HLT) to address heterogeneous multiagent problems. HLT keeps track of a pool of policies that agents have explored during training, gathering a league of heterogeneous policies to facilitate future policy optimization. Moreover, a hyper-network is introduced to increase the diversity of agent behaviors when collaborating with teammates having different levels of cooperation skills. We use heterogeneous benchmark tasks to demonstrate that (1) HLT promotes the success rate in cooperative heterogeneous tasks; (2) HLT is an effective approach to solving the policy version iteration problem; (3) HLT provides a practical way to assess the difficulty of learning each role in a heterogeneous team.

==> gen/1-intro.tex <==
\section{Introduction}
\IEEEPARstart{H}{eterogeneous}
% Heterogeneous 
multiagent reinforcement learning (HMARL) is not a new problem in MARL,
they have not yet been investigated extensively in literature.
There are many works introducing HMARL on specific domains, 
e.g. traffic control \cite{calvo2018heterogeneous}
communication \cite{fard2022time}, 
control system \cite{chen2020off}.
however, to our knowledge,
there lacks a general-purpose heterogeneous reinforcement learning algorithm,
aiming at cooperation learning within a multi-type multiagent team.

In general, classic MARL methods do not assume the type difference between agents,
nevertheless,
most existing works on MARL simply use homogeneous benchmark \cite{??} 
or heterogeneous benchmarks consisting only 2 types (e.g., most released SMAC maps \cite{??})
to claim the effectiveness their models.
However,
in reality, we live in a world of great diversity,
it is hard to find a pure homogeneous system.
Many multiagent systems require the participant of multiple agent types.

On one hand, 
ignoring heterogeneous property between agents can limit the performance of MARL models.
The non-stationary issue is one of the difficulties
presented by heterogeneous multiagent problems.
In heterogeneous multiagent tasks,
different kinds of agents var in ability, quantity,
expected functionality etc.
Notably the number of each agent type is unbalanced in most scenarios.
E.g., in military simulations,
high-value aircrafts are essential for obtaining battlefield advantage 
but are very few in number compared with ground agents.
This imparity is also common in the world of nature, 
e.g., in a hive honey bees queens and workers differ greatly in number.


On the other hand,
heterogeneous systems contain more realistic problems that has not yet been studied.
When a team of heterogeneous agents are trained and deployed,
system maintainance is still an important issue, 
which can also cost considerable resource.
When the system fails due to one of the agent type,
it is more economical to upgrade only the misbehaving agents 
rather than the whole team.
This requires agents to have the capability to 
act according to different versions of policies.
Such capability is especially essential in systems that cannot enable OTA (Over-the-Air Programming)
due to reliability or security concerns (such as military robot systems),
or systems that cannot afford to suffer a full stop in long term service 
(such as traffic and network devices).
In this work, we summarize above problems as the policy iteration problem.


In this paper, our contribution is as follows:
1. We propose Heterogeneous League Training, 
a general-purpose MARL algorithm for heterogeneous multiagent tasks.
2. We demonstrate the superior performance of HLT and the effectiveness of HLT against the policy iteration problem.
3. Based on HLT, we put forward a method to diagnose the difficult of learning the roles of each agent types.
4. We introduce UHMP (UnrealEngine-based Hybrid Multiagent Platform) as heterogeneous multiagent benchmark for 
performance evaluation.





Some misplaced content ??????????????????


% type A -> type B transfer
Nevertheless, 
due to the great difference between different types agents,
the policy cannot be generalized from one type to another.

% 加剧了Non-stationary问题


The unbalanced number of agents leads to
more inaccurate state value estimation for agents that are few in number,
compared with other agents. % put forward theory, then start explaining
In MARL agents learn from samples collected 
via interacting with the environment.
Unlike homogeneous multiagent tasks,
agents belonging to different types cannot share their experience.
For example, a patrol UAV cannot share its experience with
a ground agent since they do not have the same ability and functionality,
and they may even have different available action space.
As a result,
agents with numerious same-type companions
are likely to learn faster and establish more precise
estimation concerning their situation, 
while agents with very few same-type partners (or no partners at all)
develop their knowledge much more slowly.
% As a consequence,
% some agents will learn faster than others,
This disordered and uncoordinated learning process 
will further aggravate non-stationary of 
agents perception towards environment,
causing issues in MARL learning efficiency.

% Heterogeneous多体问题是真实世界的映射，真实世界中的不稳定性问题
As a saying goes, no two snowflakes are alike ??
There is no absolute homogeneous cooperation game in the world of nature.
Also, considering cost and reliability, homogeneous robot system 
is usually better than homogeneous systems in artificial systems.
Studying the cooperation between heterogeneous agents
bring us one step closer to applying reinforcement learning to
real world applications.

One of the gaps between reality and MARL theory is that
the policy version iteration problem.
In a heterogeneous systems,
different types of machine agents are likely manufactured by
different companies at different time.
In reality, after put into use,
we may still need to update the hardware of agents and then 
train them to adapt the updated hardware according to new requirements, 
one type of agents at a time.
A problem arises is that
updated agents with new policies may not be able to cooperate with 
other types of old agents with old policies, and vice versa.
Although we can update the policy of all types of agents easily in simulations,
in reality it can cost a lot to stop machine agents in production.

Therefore, a method to iterate policies without breaking the compatibility 
between different heterogeneous agents
is needed in order to actually apply the multiagent systems to application.


==> gen/2-rel.tex <==
\section{Related Works}

Although heterogeneous multiagent reinforcement learning (HMARL) is not a new problem in MARL,
they have not yet investigated extensively in literature.
While there are works introducing HMARL on specific domains, 
e.g. traffic control \cite{calvo2018heterogeneous}
communication \cite{fard2022time}, 
control system \cite{chen2020off}.
As far as we known,
a general-purpose heterogeneous reinforcement learning is absent.

On the other hand,
classic MARL methods ignores the type distinction between agents 
and solely depends on agent observation to 
address the type identity problem in tasks involving heterogeneous agents.




% % type A -> type B transfer
% Nevertheless, 
% due to the great difference between different types agents,
% the policy cannot be generalized from one type to another.

% % 加剧了Non-stationary问题
% % Unlike homogeneous multiagent tasks,
% The non-stationary issue is one of the difficulties
% presented by heterogeneous multiagent problems.
% In heterogeneous multiagent tasks,
% different kinds of agents var in ability, quantity,
% expected functionality etc.
% Notably the quantity of each agent type is unbalanced in most scenarios.
% E.g., in military simulations,
% high-value aircrafts are essential for obtaining battlefield advantage 
% but are very few in number compared with ground agents.
% This imparity is also common in the world of nature, 
% e.g., in a hive honey bees queens and workers differ greatly in number.

% The unbalanced number of agents leads to
% more inaccurate state value estimation for agents that are few in number,
% compared with other agents. % put forward theory, then start explaining
% In MARL agents learn from samples collected 
% via interacting with the environment.
% Unlike homogeneous multiagent tasks,
% agents belonging to different types cannot share their experience.
% For example, a patrol UAV cannot share its experience with
% a ground agent since they do not have the same ability and functionality,
% and they may even have different available action space.
% As a result,
% agents with numerious same-type companions
% are likely to learn faster and establish more precise
% estimation concerning their situation, 
% while agents with very few same-type partners (or no partners at all)
% develop their knowledge much more slowly.
% % As a consequence,
% % some agents will learn faster than others,
% This disordered and uncoordinated learning process 
% will further aggravate non-stationary of 
% agents perception towards environment,
% causing issues in MARL learning efficiency.

% % Heterogeneous多体问题是真实世界的映射，真实世界中的不稳定性问题
% As a saying goes, no two snowflakes are alike.
% There is no absolute homogeneous cooperation game in the world of nature.
% Also, considering cost and reliability, homogeneous robot system 
% is usually better than homogeneous systems in artificial systems.
% Studying the cooperation between heterogeneous agents
% bring us one step closer to applying reinforcement learning to
% real world applications.

% One of the gaps between reality and MARL theory is that
% the policy version iteration problem.
% In a heterogeneous systems,
% different types of machine agents are likely manufactured by
% different companies at different time.
% In reality, after put into use,
% we may still need to update the hardware of agents and then 
% train them to adapt the updated hardware according to new requirements, 
% one type of agents at a time.
% A problem arises is that
% updated agents with new policies may not be able to cooperate with 
% other types of old agents with old policies, and vice versa.
% Although we can update the policy of all types of agents easily in simulations,
% in reality it can cost a lot to stop machine agents in production.

% Therefore, a method to iterate policies without breaking the compatibility 
% between different heterogeneous agents
% is needed in order to actually apply the multiagent systems to application.


% \section{Heterogeneous MARL}
% A heterogeneous MARL task can be described as a Dec-POMDP \cite{oliehoek2016concise},
% which can be formulated by 
% $\langle A, \varDelta, \mathcal{U}, \mathcal{S}, P_t, \mathcal{Z}, P_o, r , \gamma\rangle$,
% where $A$ is the collection of agents and $N=|A|$ is the total number of agents.
% $\mathcal{U}$ is a collection of actions within which each agent $a_i$ can choose from.
% $\mathcal{S}$ is the set of environment states and $P_t$ is the transition function.
% $r$ is team reward. $\gamma$ is the discount factor.
% In a heterogeneous system, 
% $\varDelta = \lbrace \delta_1, \dots, \delta_{n_j} \rbrace$ is the set of agent types and 
% $n_j = |\varDelta|$ is the total number of types in the system.
% Each agent $a_i$ is categorized into a type $\text{Type}(a_i) = \delta_j$.
% Although the quantity of agents can be large,
% the the number of types is very limited $n_j \ll N$,
% since in the real world
% agents (usually robots) 
% are usually manufactured via standardized production to reduce cost.




% \section{Method}

% \subsection{League Training}
% League training is first introduced in AlphaStar \cite{vinyals2019grandmaster}.
% To effectively improve agents' initial capability,
% AlphaStar takes advantage of human expert data to train agents with a supervised approach,
% obtaining a population of agents with different policies.
% Agents are subsequently trained with reinforcement learning,
% and intermittently duplicate themselves and freeze these duplications as past players.
% The agent players are trained against each other as well as themselves in history.
% AlphaStar agent was rated at Grandmaster level in Starcraft game.

% % The significant advantage of league training is that 
% % it enables agent to learn adaptive policies which considers the different strategies of opponents.
% League training enables agents to learn adaptive and robust policies against 
% continually developping strategies of other fellow agents,
% which also has great value in heterogeneous MARL in order to 
% solve the policy iteration problem and to improve model performance.

% Unfortunately, league training cannot be applied to heterogeneous MARL because of following reasons.
% First and most importantly,
% heterogeneous agents collaborate instead of competing in heterogeneous MARL.
% (If there are two or more adversarial teams, a unit entity is refered to as an agent only in its own team).
% Secondly,
% there will be no human data for supervised pre-training.
% Thirdly,
% League training used by \cite{vinyals2019grandmaster} consumes huge amount of computational resource and 
% it will be too expensive to be applied elsewhere.

% \subsection{Heterogeneous League Training Framework}
% \subsubsection{League Collaborating Hyper Network}
% Cooperating with a variety of partners with different policies is challenging.
% Some partners are well-trained and willing to cooperate,
% while some partners using past policies frozen at not-trained states can only behave randomly.
% It is necessary to equip agents with a neural network structure 
% that is sensitive to the differences of heterogeneous partners.

% For a heterogeneous team with agents $\lbrace a_1, \dots, a_{N} \rbrace$,
% we use a tuple $\langle \alpha,  \rangle$
% \begin{equation}

% \end{equation}

% describe the 
% aware of
% A hyper-network structure to solve the conflicts of cooperating with 
% different versions of agent partners.



% To

% By making agent players competing with others and themselves in history,
% eventually overcome continually adapting strategies.


% which spawns a great population of player agents.
% we 

% Traditionally,
% when training a multiagent systems


% If we can find a way to iterate policies 
% without breaking the compatibility between different types of agents,

% To finish such updates a problem must be solved.

% it is    a hardware update or 

% it is common for human operators to spot flaws

% it may be inconvenient or impossible to replace

% different types of agents are manufectured by different

% One of the concern arise in homogeneous systems






% For example,
% many methods use attention mechanism to process large observation space,
% but different types of agents may have to learn distinct ways to
% pay attention diff

==> gen/3-prelim.tex <==
\section{Preliminaries}
\subsection{Heterogeneous MARL.}
A heterogeneous MARL task can be described as a Dec-POMDP \cite{oliehoek2016concise},
which can be formulated by 
$\langle A, \varDelta, \mathcal{U}, \mathcal{S}, P_t, \mathcal{Z}, P_o, r , \gamma\rangle$,
where $A$ is the collection of agents and $N=|A|$ is the total number of agents.
$\mathcal{U}$ is a collection of actions within which each agent $a_i$ can choose from.
$\mathcal{S}$ is the set of environment states and $P_t$ is the transition function.
$r$ is team reward. $\gamma$ is the discount factor.
In a heterogeneous system, 
$\varDelta = \lbrace \delta_1, \dots, \delta_{n_j} \rbrace$ is the set of agent types and 
$n_j = |\varDelta|$ is the total number of types in the system.
Each agent $a_i$ is categorized into a type $\text{Type}(a_i) = \delta_j$.
Although the quantity of agents $N$ can be large,
the the number of types $n_j$ is considerably smaller ($n_j \ll N$),
this is because in the real world agents (usually robots) 
are usually manufactured via standardized production to reduce cost.
Furthermore, considering the cost,
it is common that agents of high-value types are lesser in number 
than cheap agents in a functional heterogeneous team.

\subsection{League Training in AlphaStar.}
League training is first introduced in AlphaStar \cite{vinyals2019grandmaster}.
To effectively improve agents' initial capability,
AlphaStar takes advantage of human expert data to train agents with a supervised approach,
obtaining a population of agents with different policies.
Agents are subsequently trained with reinforcement learning,
and intermittently duplicate themselves and freeze these duplications as past players.
The agent players are trained against each other as well as themselves in history.
The trained AlphaStar agent was rated at Grandmaster level in Starcraft game.

% The significant advantage of league training is that 
% it enables agent to learn adaptive policies which considers the different strategies of opponents.
League training enables agents to learn adaptive and robust policies against 
continually developping strategies of other fellow agents,
which also has great value in heterogeneous MARL in order to 
solve the policy iteration problem and to improve model performance.

Unfortunately, league training cannot be applied to heterogeneous MARL because of following reasons.
First and most importantly,
heterogeneous agents collaborate instead of competing in heterogeneous MARL.
(If there are two or more adversarial teams, a unit entity is refered to as an agent only in its own team).
Secondly,
there will be no human data for supervised pre-training.
Thirdly,
League training used by \cite{vinyals2019grandmaster} consumes huge amount of computational resource and 
it will be too expensive to be applied elsewhere.



==> gen/4-hlt.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%Heterogeneous League Training%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Heterogeneous League Training}

\begin{figure}[!t]
  \centering
  \includegraphics[width=\linewidth]{img/league-crop.pdf}
  \caption{Heterogeneous League Training framework.}
  \label{fig:main-fig}
  \end{figure}


Next, we propose a Heterogeneous League Training (HLT) algorithm motivated AlphaStar,
an efficient and general-purpose multiagent reinforcement learning algorithm for heterogeneous cooperative systems.

In this section, 
we start by stating our motivation and model features in Sec~\ref{sec:motivation}, 
e.g., our league training model is designed for promoting the ability of cooperating instead of competing.
Next,
we briefly introduce the general framework of HLT in Sec~\ref{sec:framework}.
Then,
the details of heterogeneous league training is further presented in Sec~\ref{sec:x} and Sec~\ref{sec:xx}.
Finally,
as an essential struture to achieve adaptive cooperative behaviors,
the design of hyper networks is illustrated in Sec~\ref{sec:xxx}.



\subsection{Motivation and Features.}
\label{sec:motivation}
HLT aims at two goals in heterogeneous multiagent RL:
\begin{itemize}
  \item Taking advantage of the feature of heterogeneous systems to facilitate cooperation.
  \item Addressing the policy iteration problem.
\end{itemize}

\subsubsection{Motivation.} 

Following reasons inspired us to use the league training technique to achieve our goals.
Firstly, 
different agent types vary considerably in quantity.
Samples that RL algorithm gathers from epsiodes
can provide low-variance experience for classes with numerious agents (T+),
on the other hand, 
classes with comparably fewer agents (T-) receive high-variance experience.
The learning process becomes instable when T- agents fail to catch up with the progress of T+ agents,
and T+ agents give up counting on T- agents and 
turn to develop uncooperative policies which excludes the help of T-.
By adopting the cooperative league training technique,
agents optimize their policies 
not only from the experience of cooperating with each other,
but also from the experience of teaming up with foreign agents with different cooperation skills. % (parameter-frozen) 
More specifically,
cooperative league training technique addresses the learning instability problem 
by encouraging agents to use different cooperation behaviors depending on who their teammates are.

Secondly,
cooperative league training provides an environment where
agents are trained to work with a league of heterogeneous teammates 
equipped with diverse collaboration preference.
By adding history agent policies into the league,
agents can learn new cooperative behaviors 
while not forgetting the way to collaborate with old versions of heterogeneous teammates.


\subsubsection{Key Features.} 

First and most importantly,
AlphaStar is an example of a \textbf{adversarial} multiagent league training algorithm, 
where agents are trained to compete.
What we propose in this paper is a \textbf{cooperative} league training method, 
which is designed to facilitate heterogeneous agent cooperation.

Secondly,
AlphaStar league model requires distributed servers with TPUs to run concurrent matches,
but our algorithm only needs a single machine with a single GPU 
to execute the whole training process.
To achieve this, 
we redesign the procedure of the league training based on 
the characteristic of heterogeneous systems.
Furthermore,
we introduce a hyper-network structure, 
facilitating each agent with the ability to change its cooperative behavior 
according to its type and the performance of its heterogeneous teammates.




\begin{figure*}[!t]
  \centering
  \includegraphics[width=0.8\linewidth]{img/framework-crop.pdf}
  \caption{Policy optimization cycle.}
  \label{fig:optimization}
  \end{figure*}

\subsection{Overall Framework of HLT.}
\label{sec:framework}

\subsubsection{Actors and Critic.}
Our Heterogeneous League Training (HLT) model 
follows the Centralized-Training-Decentralized-Execution (CTDE) paradigm.
Agents learn the class identities of the whole heterogeneous team from the observation,
in which each agent's class is described by a one-hot vector.
Agents belonging to the same class share the policy network parameters,
while agents from different classes can choose freely 
between using shared network parameters or using independent networks.
Therefore, 
we use a term \textbf{policy group} (denoted as $\vec{\pi}$) to describe the policy/policies
of an entire heterogeneous team.
For generality,
policies for each agent class is represented by:
$$
  \vec{\pi} = \lbrace \pi(\delta_1),\dots, \pi(\delta_M) \rbrace
$$
where $ \delta_1, \dots, \delta_{n_j} $ represent each agent class.
Note that each policy $\pi(\delta_j)$ controls all $\delta_j$ agents in the team.

The computational cost is a serious concern in cooperative multiagent systems.
Consequently, we only initia lize and optimize one dynamic policy group during league training.
This poicy group is refered to as the \textbf{frontier policy group} or $\vec{\pi}_{\text{f}}$.

We establish a policy pool refered to as a league $\mathcal{L}$ to hold history policies,
similar to AlphaStar.
As shown in Fig.\ref{fig:main-fig}, 
a series of past policies is intermittently duplicated and seperated from the frontier, 
and then placed into the past pool during training.
Once independent from the frontier,
the network parameters of past policies are frozen
so that we only need to to compute policy gradient for frontier policies 
instead of for all policies in the pool.
Those frozen policies in the league are refered to as \textbf{past policy groups}.
Let $|\mathcal{L}|$ be the total number of policies in the league,
each member policy group is denoted as:
$$\mathcal{L}=\lbrace 
\vec{\pi}_{\text{p},1}, \dots, \vec{\pi}_{\text{p},|\mathcal{L}|}
 \rbrace
$$


Additionally,
while there are different groups of policy network (as actors) in HLT,
there is \textbf{only one critic network} in HLT to action assessment during the whole training process.

\subsubsection{Optimization Iteration.}
As illustrated in Fig.~\ref{fig:main-fig},
the algorithm begins with a randomly initialized policy group and a empty league.
This group of random policies is the initial frontier policy group.
When each policy optimization iteration is done,
the new policy group (frontier) will be evaluated by a filter,
which determines whether it distinct from the policies already inside the league.
If the new frontier deviates much from policies in the league,
it will be accepted as a new member in the league.
Otherwise, the league stays unchanged till next iteration.

In each optimization iteration, 
if the league is empty,
agents directly interact with the environment with the frontier policy group,
and collect epsiode samples for initial policy optimization.
When the league contains past policy groups,
agents will randomly sample policies from both the frontier and the league
for the policy optimization.

\begin{figure*}[!t]
  \centering
  \includegraphics[width=0.8\linewidth]{img/hypernet-crop.pdf}
  \caption{Hyper network for learning adaptive cooperative behavior.}
  \label{fig:hyper}
  \end{figure*}

\subsection{League Sampler.}
\label{sec:LeagueSampler}
\label{sec:x}

As shown in Fig.~\ref{fig:optimization},
the frontier policy group is trained to cooperate not only with itself,
but also with history policies it visited previously during the learning process.

For each episode,
the league sampler randomly generate a policy combination $C_{\text{sel}}$.
This combination is either frontier-past
$C_{\text{sel}}=(\vec{\pi}_{f}, \vec{\pi}_{\text{p},l})$, 
or frontier-frontier
$C_{\text{sel}}=(\vec{\pi}_{f} , \vec{\pi}_{f})$.
The balance between frontier-frontier and frontier-past combination 
is adjusted by a constant hyper-parameter $p_f \in \left[0,1\right)$:
\begin{equation}
\begin{array}{ll}
  &P\left[C_{\text{sel}}=\left( \vec{\pi}_{f}, \vec{\pi}_{\text{p},l} \right)    \mid p_f \right] = \frac{1}{(1-p_f)|\mathcal{L}|} \\
  &P\left[C_{\text{sel}}=\left( \vec{\pi}_{f}, \vec{\pi}_{f}          \right)    \mid p_f \right] = p_f
\end{array}
\end{equation}
where $|\mathcal{L}|>0$ and $p_f<1$. 
When the league is empty ($|\mathcal{L}|=0$), 
league sampler simply provides frontier-frontier combination, 
namely $C_{\text{sel}}=( \vec{\pi}_{f}, \vec{\pi}_{f} )$.
When $p_f=0$, the sampler avoids pure frontier combination 
and always samples one of the past policy group from the league in $C_{\text{sel}}$.
On the other hand,
when $p_f \approx 1$, 
the sampler tends to exclude the participant of the league.






Next, 
a combination sampler receives $C_{\text{sel}}$ and 
eventually determines the policy that each agent executes.
For clarity, we use $\vec{\pi}_\text{sel}$ and $C_{\text{sel}} = (\vec{\pi}_f, \vec{\pi}_\text{sel} )$ to represent 
the selected policy group and the combinaiton respectively.
As shown in Fig.~\ref{fig:optimization}, 
the combination sampler choose one of the agent class to play the past policies, 
each class has equal probability to be selected,  regardless the number of agents it possesses:
$$
  P(\delta_j) = \frac{1}{|\varDelta|}, \forall \delta_j \in \varDelta
$$
Finally, with a agent type $\delta_t$ chosen to use the corrisponding policy in group $\vec{\pi}_\text{sel}$.
The mix policy group $\vec{\pi}_{\text{mix}}$ that the team executes is:
$$
  \vec{\pi}_{\text{mix}} = \lbrace \pi_{\text{mix}}(\delta_1),\dots, \pi_{\text{mix}}(\delta_M) \rbrace
$$
where
$$
    \pi_{\text{mix}}(\delta_j) = \left\{\begin{array}{ll}
        \pi_f(\delta_j),            & \delta_j \neq  \delta_t \\
        \pi_{\text{sel}}(\delta_j), & \delta_j = \delta_t
    \end{array}\right., \forall \delta_j \in \varDelta
$$

The mix policy group $\vec{\pi}_{\text{mix}}$ only influences one episode.
But the league sampler and combination sampler can generate 
a batch of different $\vec{\pi}_{\text{mix}}$ to run in parallel.
This process is repeated to collect a batch of episodes for frontier policy optimization.
The policy gradient w.r.t. the frontier policy parameters is calculated from the collected episodes,
and used to optimize each frontier policy of each agent type.


  
\subsection{League Member Management.}
\label{sec:LeagueManagement}
\label{sec:xx}
To be able to run on a single machine, HLT has to control the size of the league. 
In AlphaStar, researchers use a large past agent pool which cost a significant amount of memory and time,
which is not applicable in most heterogeneous problems.
From the intuition that the league should contain policies with diverse behaviors and distinct cooperative ability,
we use a league filter to manage and control the league size as shown in Fig.\ref{fig:optimization}.

In HLT a metric $\Omega \in [0,1]$ is introduced to compare the similarity of policy groups.
This metric can be the success rate, normalized test reward 
(projecting the minimum reward and maximum reward to 0 and 1 respectively),
or any other evaluation scores that reflect policy performance.

Let $|\mathcal{L}|_{\text{max}}$ be the maximum size of the league.
if the size of the pool is exceeds $|\mathcal{L}|_{\text{max}}$,
the league filter deals with policy group candidates using following procedures:
\begin{itemize}
\item (1) evaluate the new policy group with metric $\Omega$.
\item (2) add the policy group into the league.
\item (3) sort all policy groups in the league according to their $\Omega$ metric.
\item (4) the league filter finds a pair of policy groups with closest evaluation metric, and then remove the newer group.
\end{itemize}


More specifically, since the league capacity is exceeded during step (2)\~(4):
$$\mathcal{L}=\lbrace \vec{\pi}_{\text{p},1}, \dots, \vec{\pi}_{\text{p},|\mathcal{L}|+1}  \rbrace$$
to find a policy group to remove, 
we first evaluate each past policy group with  metric $\Omega$:
$$
\Omega(\mathcal{L}) = \left\lbrace   \Omega(\vec{\pi}_{\text{p},1}), \dots,    \Omega(\vec{\pi}_{\text{p},|\mathcal{L}|+1})     \right\rbrace = \lbrace \omega_1, \dots, \omega_{|\mathcal{L}|_{\text{max}}+1} \rbrace
$$
where $\omega_1, \dots, \omega_N, \omega_{|\mathcal{L}|_{\text{max}}+1}$ are evaluation scores.
Then the league is sorted according to $\omega$ scores,
rearranging $\mathcal{L}$ so that:
$$
\omega_1 \le \dots \le \omega_N \le \omega_{|\mathcal{L}|_{\text{max}}+1}
$$
Finally, find a pair of policy groups $\vec{\pi}_{\text{p},k}$ and $\vec{\pi}_{\text{p},k+1}$ with closest evaluation metric:
$$
     |\omega_{k+1} - \omega_{k} | \le |\omega_{k'+1} - \omega_{k'} |, \quad \forall k' \in [1, |\mathcal{L}|_{\text{max}}]
$$

Then the order of when group $k$ and group $k+1$ are added into the pool is considered,
we always remove the newer policy group within $\vec{\pi}_{\text{p},k}$ and $\vec{\pi}_{\text{p},k+1}$.
By removing the relatively newer group instead of the older group,
we can avoid frequent changes taking place inside the league and prevent potiential instability.
After removal the size of league reduces back to $|\mathcal{L}|_{\text{max}}$.

\subsection{Adaptive Hyper Network.}
\label{sec:hyper}
\label{sec:xxx}
% Cooperating with a variety of partners with different policies is challenging.
% Some partners are well-trained and willing to cooperate,
% while some partners using past policies frozen at not-trained states can only behave randomly.
% It is necessary to equip agents with a neural network structure 
% that is sensitive to the differences of heterogeneous partners.


Cooperating with a variety of partners with different policies is challenging.
For any type of agents,
they may encounter strong partners that are well-trained and cooperative,
on the other hand,
they may also meet weak partners using past policies frozen at immature stages.
It is necessary to equip agents with a neural network structure 
that is sensitive to the differences of heterogeneous partners.
In HLT, 
we use a hyper-network structure to achieve this goal.

As shown in Fig.~\ref{fig:hyper}, 
the hyper-network is a structure to generate network parameters for MLP layers in the main policy network.
Internally, 
the hyper-network uses 2 layers of fully connected network to produce MLP parameters,
using a agent-team information vector $F_h$ as input.

The agent-team information vector $F_h$ is determined by agent class $\delta_j$ and the mix policy $\vec{\pi}_{\text{mix}}$. 
It is a concatenation two parts:
$$
F_h(\delta_j, \vec{\pi}_{\text{mix}}) = \operatorname{concat}\left[ \ 
    F_{v}(\delta_j, \vec{\pi}_{\text{mix}}) 
    , \ 
    F_{\delta}(\delta_j) \  
    \right]
$$
$F_{\delta}$ is a one-hot binary vector for the distinction of agent classes. 
E.g, if $\delta_j=\delta_1$, then $F_{\delta}(\delta_j)=F_{\delta}(\delta_1)=[1, 0, 0, \dots]$.
And $F_{v}(\delta_j, \vec{\pi}_{\text{mix}})$ represents the combination of the mixed heterogeneous team 
by identifying the policy that each agent class executes. 
$$
    F_{v}(\delta_j, \vec{\pi}_{\text{mix}})  = (V_{\delta_1},\dots,V_{\delta_{|\varDelta|}})
$$

$$
    V_{\delta_j}=\left\{\begin{array}{ll}
            1,                                      & \delta_j \neq  \delta_\text{sel} \\
            \Omega[\pi_{\text{sel}}(\delta_j)],     & \delta_j = \delta_\text{sel}
    \end{array}\right., \quad \forall \delta_j \in \varDelta
$$
where $V_{\delta}$ describes frontier policies with constant $\Omega_\text{max}= 1$ and past policies with the metric $\Omega$ of their policy group.
Since $\Omega[\pi_{\text{sel}}(\delta)] < 1$ before the completion of training,
$V_{\delta}$ always illustrates the difference between frontier policies and past policies.

Specially,
we also need to consider the hyper-network input for past policies.
As mentioned previously,
all past policies are duplications of the frontier policy at a certain stage,
they, same as the frontier policy, were always trained under the circumstance 
where they observe themselves as the frontier, i.e. $V_{\delta} = 1$.
For consistency, 
past policies still observe themselves as frontiers with $V_{\delta}=1$.
Concretely,
differing from $F_h$,
past policies use $\hat{F}_h$ as hyper-network input:
$$
\hat{F}_h(\delta_j, \vec{\pi}_{\text{mix}}) = \operatorname{concat}\left[ \ 
    [1,1,\dots,1]
    , \ 
    F_{\delta}(\delta_j) \  
    \right]
$$

Afterwards, the hyper-network produces a vector of parameters $\theta_h$:
$$
\theta_h = \text{HyperNet}(\hat{F}_{v})
$$
Two MLP layers are used as the struture of the hyper-network.
Then vector $\theta_h$ is split and reshaped 
into weight matrix $w_h$ and bias vector $b_h$,
which work as feed forward layers $f$ in the main policy network:
$$
    f( h | \theta_h) = \text{Relu} (w_h h + b_h)
$$
where $h$ represents the input of the network layers.



% For a heterogeneous team with agents $\lbrace a_1, \dots, a_{N} \rbrace$,
% we use a tuple $\langle \alpha,  \rangle$
% \begin{equation}

% \end{equation}

% describe the 
% aware of
% A hyper-network structure to solve the conflicts of cooperating with 
% different versions of agent partners.


==> gen/5-exp.tex <==
\section{Experiments}


\begin{figure}[!t]
  \centering
  \includegraphics[width=0.6\linewidth]{img/uhmp-f1-crop.pdf}
  \caption{A map of Unreal-based Hybrid Multiagent Platform (UHMP), 
  with 2 support UAVs and 8 ground agents on each side.}
  \label{fig:uhmp-f1}
  \end{figure}

\begin{figure}[!t]
  \centering
  \includegraphics[width=0.5\linewidth]{img/uhmp-f3-crop.pdf}
  \caption{ An illustration of supportive UAV agents.
  Supportive UAV agents (Type 1) are responsible to repair and assist nearby agents, 
  equipped with missile-weapon payload but are vulnerable to opponent attacks.
  }
  \label{fig:uhmp-f3}
  \end{figure}
      

\begin{figure}[!t]
  \centering
  \includegraphics[width=0.5\linewidth]{img/uhmp-f2-crop.pdf}
  \caption{An illustration of two types of ground agents. 
  Agents of the second type (Type 2) are ground units with missile-weapon payload.
  Agents of the third type (Type 3)  are ground units with kinetic-weapon payload.
  }
  \label{fig:uhmp-f2}
  \end{figure}


  
\subsection{Heterogeneous Benchmark Environment.}
The heterogeneous league training algorithm is tested under
the Unreal-based Hybrid Multiagent Platform (UHMP),
an advanced heterogeneous simulation environment.
As shown in Fig.\ref{fig:uhmp-f1} and Fig.\ref{fig:uhmp-f3},
we use a built-in AI as the opponent of the HMARL learner,
two teams share symmetrically configurations.
Moreover, 
we use tags such as \text{2u-4m-4k} and \text{2u-4m-14k} to represent the configurations.
E.g.,
the sequence \text{2u-4m-4k} indicates the type and number of heterogeneous agents in each team.
Each team has 2 supportive air-borne UAV agents ($\delta_1$, \text{2u}), 
capable of attacking, 
repairing allies and reducing damage caused by opponents.
The other 8 agents are ground units.
Half of them have missile-weapon payload and long attack range ($\delta_2$, \text{4m}).
Other ground units ($\delta_3$, \text{4k}) equip kinetic weapons with short attack range,
and are incapable of attacking opponent UAVs.
$\varDelta = \lbrace \delta_1, \delta_2, \delta_3 \rbrace$ and $|\varDelta| = 3$.

The functionality of different agents in UHMP is also shown in Fig.\ref{fig:uhmp-f2} and Fig.\ref{fig:uhmp-f2}.
Due to the ability difference,
agents belonging to one type have to learn policies 
that are, to an extent, unshareable to other heterogeneous types.
Furthermore,
due to the imparity of quantity between different types,
the importance and learning difficulty of agent types diverges from one another.


\subsection{Algorithm Performance Evaluation.}
\subsection{Experimental Setup.}

We run our experiments on a single linux server with regular AMD CPUs and Nvidia GPUs (RTX 8000),
and we only use one GPU for each experiment.
PPO and Adam optimizer is used for applying policy gradient on policies neural networks.
We adopted dual-clip PPO and policy resonance technique to improve training efficiency.
To control the involvement of the league,
we set $p_f=0.1$ for the league sampler by default,
so that in 90\% of all episodes,
agents executes mixed policies with the participant of both frontier and past policies.
We set $|\mathcal{L}|_\text{max} = 5$ due to the consideration 
that running a large number of past policy group concurrently 
can significantly slow down the model calculation.
During we frequently evaluate the frontier policy group with winning rate as the metric $\Omega$,
for precision we run 160 episodes in every evaluation,
the intermittent evaluation takes place once every 1600 training episodes.
In experiments, we run each experiment settings repeatedly with at least 4 different random seeds.


\subsection{Performance of HLT.}
To test the effectiveness of the proposed HLT model,
we compare proposed HLT method with existing SOTAs 
such as FT-Qmix (fine-tuned Qmix) \cite{?}.

While individual observations alone suffice the need of HLT,
some of the those method such as Qmix requires an extra state information vector 
during centralized training.
Determining how the additional states is obtained,
we use '-D' suffix to represent a model trained 
in a Delicately designed state space,
or no suffix to represent a model trained 
in an untuned state space (or not using state information at all).



% We investigate how
% We examine whether both chosen motivational indices are essential.
% (a) We assess how the concentration parameter dc influences the module. 
% (b) We investigate whether the extra
% self-attention layer shown in Fig. 1 provides improvement.
% (c) We examine whether reducing our model from DualConcNet to Single-ConcNet causes a performance decay.
% (d) We investigate whether Conc-4Hist model can ultilize
% history observations under extreme interference.

\subsection{The Effectiveness Against Policy Iteration Problem.}
\label{PolicyIteration}
We investigate how HLT model improves the policies compatibility 
between different versions of policies.
When the trainning is completed,
we test whether a fully trained policy group (the eventual frontier policy group) 
can promote the win rate of past policies when mixed together.
In this test,
we still use the random combination sampler introduced previously 
for following tests of frontier-past policy compatibility:
\begin{itemize}
  \item For each episode, randomly select one type of agents that executes the past policies, 
    while the types of agents execute the frontier policies. (Frontier exclusive test.)
  \item For each episode, Randomly select one type of agents that executes the frontier policies, 
    while the types of agents execute the past policies. (Frontier inclusive test.)
  \end{itemize}


In the former test, 
frontier policy group controls most types of agents.
With the frontier policy group being the majority in the team, 
we assess how the frontier work with the minority of agents 
controlled by past policies with various cooperation capabilities.
In the latter test,
we examine how the frontier policies response to a scenerio where
most agents are using past policies.
Playing a minority type in the heterogeneous team without dominant position,
this challenges the frontier's capability to adapt.

\subsection{Investigation on Heterogeneous Role Learning.}
In policy iteration test, 
we sample the type combination randomly and 
only focus on the frontier's adaptive ability as a group.
However,
it is also valuable to investigate the difference 
between frontier policies (which control different types of agents).
This experiment provides us a way to assess the difficulty of 
learning each heterogeneous roles,
and furthermore offer a new perspective for
analyzing how a cooperative heterogeneous 
joint policy comes into existance.



\section{Results.}

\subsection{Main Results.}
We compared our HLT method with other SOTAs on two main common metric, 
namely win rate and test reward.
Each score is averaged over 160 test episodes, 
and then averaged again over 
at least 4 independent experiments launched by different random seeds.

\begin{table}[!t]
  \centering
  \setlength{\tabcolsep}{0.5mm}{
    \begin{tabular}{ccc}
      \toprule
      {Algorithm} 
                                      & {Best Test Win Rate}  
                                                              & {Best Test Reward}         \\
      \midrule
      {HLT         }  
                                      & \textbf{98.09\%}              
                                                              & \textbf{1.782}      \\
      {FineTuned Qmix} 
                                      & {87.98\%}              
                                                              & {1.452}   \\
      {FineTuned Qmix-D}              
                                      & {91.79\%}              
                                                              & {1.547}   \\
      \bottomrule
  \end{tabular}
  }
  \caption{
    Performance comparison between methods.
  }
  \label{table:performance}
\end{table}
From the results shown in Fig.\ref{table:performance},
HLT has the best performance among all models 
despite that HLT does not use any state information.
FineTuned Qmix also has relatively good performance 
when trained by delicately designed global state.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Heterogeneous Cooperation Policy.}

Observating the finalized policies trained by HLT,
we find a clear agent role division between different agent types.
Fig.\ref{fig:uhmp} demonstrates a scenerio where 
green RL agents preparing to contact the enemy.
T1 agents (UAVs) take advantage of its agility 
by moving back and forth 
to attack enemies and simultaneously support ground teammates.
T2 agents has longer attack range than T3,
but they learned a hit-and-run policy,
moving ahead of T3 agents when opponents is far but 
immediately retreat behind T3 agents when facing threats.
The strengh of T3 agents is short range combat,
but being in a heterogeneous team they learn
a rather sedate policy, 
which stays still when simulation begins
and then forms a circle formation along with T2 when opponents approach.





\begin{figure*}[!t]
  \centering
  \begin{subfigure}[t]{0.32\linewidth}
  \centering
  \includegraphics[width=\linewidth,height=0.6\linewidth]{uhmp/s1.jpg}
  \caption{Step 4. T2 advancing.}
  \label{fig:dca1}
\end{subfigure}
%  
\begin{subfigure}[t]{0.32\linewidth}
  \centering
  \includegraphics[width=\linewidth,height=0.6\linewidth]{uhmp/s2.jpg}
  \caption{Step 8. T3 advancing.}
  \label{fig:dca2}
\end{subfigure}
%  
\begin{subfigure}[t]{0.32\linewidth}
  \centering
  \includegraphics[width=\linewidth,height=0.6\linewidth]{uhmp/s3.jpg}
  \caption{Step 11. Circle formation.}
  \label{fig:dca3}
\end{subfigure}
%  
\caption{Cooperating with clear role division, HMARL algorithm controls green team, 
and the opponents are represented with blue color.
The moving direction of agents is represented by circles and red arrows nearby each agent in figures.}
\label{fig:uhmp}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Policy Compatibility.}

Fig.\ref{fig:win_rate_absolute_improvement_both}
demonstrates the win rate improvement when
the frontier policy group interferes the past policy groups.
The past policy groups have different levels of cooperative ability,
quantified by their $\Omega$ metric (independent win rate).
We use past policy groups with $\Omega < 0.90$,
which are more distinguishable from the frontier policy group with $\Omega \approx 1$.
We use two kinds of test described in Sec~\ref{PolicyIteration},
frontier exclusive test results are represented by blue samples,
and frontier inclusive test results are shown with red samples.
A significant improvement can be observed for policy group 
with $\Omega \in (0.2, 0.6)$ in both tests,
the participance of the eventual frontier policy promotes 
the win rate notablely above the green $\Omega$ baseline,
this suggests an affinity can be established between the frontier and those past policies.
When $\Omega > 0.7$, 
the room for improvement is very limited,
but in most experiments frontier policies can still provide compatibility for those policies 
without raising conflicts that ruins the cooperation win rate.



\begin{figure}[h]
  \centering
  \includegraphics[width=0.6\linewidth]{img/win_rate_absolute_improvement_both.pdf}
  \caption{Compatibility between finalized policies and past policies. 
  Win rate with the participant of eventual frontier policies.}
  \label{fig:win_rate_absolute_improvement_both}
\end{figure}


% \begin{figure}[h]
%   \centering
%   \includegraphics[width=0.6\linewidth]{img/win_rate_improvement_both.pdf}
%   \caption{Compatibility between finalized policies and past policies. 
%   Improvement with the participant of eventual frontier policies.
%   }
%   \label{fig:PolicyIteration}
% \end{figure}


\begin{figure}[h]
  \centering
  \includegraphics[width=0.6\linewidth]{img/win_rate_improvement_both.pdf}
  \caption{A wrong images.}
  \label{fig:win_rate_improvement_both}
\end{figure}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Heterogeneous Role Learning.}
\begin{figure}[h]
  \centering
  \includegraphics[width=0.6\linewidth]{img/ReplaceTest1.pdf}
  \caption{Revealing heterogeneous role learning process 
  by mixing the frontier and the past policies. (Frontier exclusive.)}
  \label{fig:ReplaceTest1}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.6\linewidth]{img/ReplaceTest2.pdf}
  \caption{Revealing heterogeneous role learning process 
  by mixing the frontier and the past policies. (Frontier inclusive.)}
  \label{fig:ReplaceTest2}
\end{figure}

Every types of agents are important in a heterogeneous task.
However,
the fact that different roles that agents learn vary in difficulty.
With HLT model,
we can investigate and track the learning process of individual agent types.

The role learning process can be evaluated from two different aspects.
Fig.\ref{fig:ReplaceTest1} reveals the decline of win rate 
when one of the agent types turn to execute past policies 
instead of the eventual frontier policy.

When $\Omega \approx 0$,
the past policies back then are almost random.
At this point, 
replacing the policy of T1 (UAVs) 
causes most serious consequences (reducing win rate by 90\% on average),
while the influence of replacing the policy of T2 is relatively smaller.
This suggests that well functioning T1 agents 
are most indispensable in the frontier policies compared with other two agent types.
Nevertheless, T1 agents catch up fast with other agents 
when the policy group reaches $\Omega \approx 0.4$.
On the other hand,
T3 agents have the slowest win rate ascent among all three agent types,
and frequently becomes the black sheep after team $\Omega > 0.4$.
This indicates that the policy of T3 is usually the most difficult policy to learn.
However,
we also point out that the role learning process is sophisticated,
the conclusion on the indispensability and learning difficult of agent types 
is only based on statistics and may not stand in individual cases.
E.g., there are some individual experiment samples that are outliers,
indicating a different situation 
is encountered in those particular training process. 

% we also noticed that this result has high variance in Fig.\ref{fig:ReplaceTest1},
% in some individual experiments,
% we 

% This does not suggests the difficulty of roles.


















% HLT和其他方法的胜率对比

% HLT和不使用HLT前后，策略兼容性对比

% HLT策略兼容性的进一步研究，定量化地展示每一个类别智能体对任务的重要性


==> gen/6-conclusion.tex <==


\section{Conclusions}
In this work, 
we propose a general-purpose multiagent reinforcement algorithm
for addressing heterogeneous multiagent problems.



==> tex_bk/1-intro.tex <==
\section{Introduction}
% 缺少通用性HMARL算法 
% \IEEEPARstart{H}{eterogeneous}
Heterogeneous Multiagent Reinforcement Learning (HMARL) is not a new problem in MARL,
they have not yet been investigated extensively in the literature.
There are many works introducing HMARL on specific domains, 
e.g. 
communication \cite{fard2022time} and UAV allocation \cite{zhao2019fast}.
however, to our knowledge,
there lacks a general-purpose heterogeneous reinforcement learning algorithm,
aiming at cooperation learning within a multi-type multiagent team.

% 一般MARL算法, 异构性不足
In general, classic MARL algorithms do not assume the type difference between agents,
nevertheless,
most existing works on MARL primarily focus on homogeneous environments \cite{zheng2018magent, deka2021natural, fu2022concentration} 
or heterogeneous benchmarks consisting of only 2 types (e.g., most SMAC maps \cite{samvelyan2019starcraft})
to claim the effectiveness of their models.
However,
in reality, we live in a world of diversity,
it is hard to find a pure homogeneous system.
Many multiagent systems require the participation of multiple agent types.

% 缺点
On one hand, 
ignoring heterogeneous properties between agents can limit the performance of MARL models.
The non-stationary issue is one of the difficulties
presented by heterogeneous multiagent problems.
In heterogeneous multiagent tasks,
different kinds of agents vary in ability, quantity,
expected functionality etc.
Notably, the number of each agent type is unbalanced in most scenarios.
E.g., in military simulations,
high-value aircraft are essential for obtaining battlefield advantage 
but are very few in number compared with ground agents.
This imparity is also common in the world of nature, 
e.g., in a hive, honey bee queens and workers differ significantly in number.


% 缺点
On the other hand,
heterogeneous systems contain more realistic problems that have not yet been studied.
When a team of heterogeneous agents is trained and deployed,
system maintenance is still an important issue, 
which can also cost considerable resources.
When the system fails due to one of the agent types,
it is more economical to upgrade only the misbehaving agents 
rather than the whole team.
This requires agents to have the capability to 
act according to different versions of policies.
Such capability is especially essential in systems that cannot enable OTA (Over-the-Air Programming)
due to reliability or security concerns (such as military robot systems),
or systems that cannot afford to suffer a full stop in long-term service 
(such as traffic and network devices).
Therefore, a method to iterate policies without breaking the compatibility 
between different heterogeneous agents
is needed to apply the learned RL policies to actual applications.
In this work, we summarize the above problems as the policy iteration problem.

% 贡献
In this paper, our contribution is as follows:
1. We propose Heterogeneous League Training, 
a general-purpose MARL algorithm for heterogeneous multiagent tasks.
2. We demonstrate the superior performance of HLT and the effectiveness of HLT against the policy iteration problem.
3. Based on HLT, we put forward a method to diagnose the difficulty of learning the roles of each agent type.
4. We introduce UHMP (UnrealEngine-based Hybrid Multiagent Platform) as the heterogeneous multiagent benchmark for 
performance evaluation.





% Some misplaced content ??????????????????


% % type A -> type B transfer
% Nevertheless, 
% due to the great difference between different types agents,
% the policy cannot be generalized from one type to another.

% % 加剧了Non-stationary问题


% The unbalanced number of agents leads to
% more inaccurate state value estimation for agents that are few in number,
% compared with other agents. % put forward theory, then start explaining
% In MARL agents learn from samples collected 
% via interacting with the environment.
% Unlike homogeneous multiagent tasks,
% agents belonging to different types cannot share their experience.
% For example, a patrol UAV cannot share its experience with
% a ground agent since they do not have the same ability and functionality,
% and they may even have different available action space.
% As a result,
% agents with numerious same-type companions
% are likely to learn faster and establish more precise
% estimation concerning their situation, 
% while agents with very few same-type partners (or no partners at all)
% develop their knowledge much more slowly.
% % As a consequence,
% % some agents will learn faster than others,
% This disordered and uncoordinated learning process 
% will further aggravate non-stationary of 
% agents perception towards environment,
% causing issues in MARL learning efficiency.

% % Heterogeneous多体问题是真实世界的映射，真实世界中的不稳定性问题
% As a saying goes, no two snowflakes are alike ??
% There is no absolute homogeneous cooperation game in the world of nature.
% Also, considering cost and reliability, homogeneous robot system 
% is usually better than homogeneous systems in artificial systems.
% Studying the cooperation between heterogeneous agents
% bring us one step closer to applying reinforcement learning to
% real world applications.

% One of the gaps between reality and MARL theory is that
% the policy version iteration problem.
% In a heterogeneous systems,
% different types of machine agents are likely manufactured by
% different companies at different time.
% In reality, after put into use,
% we may still need to update the hardware of agents and then 
% train them to adapt the updated hardware according to new requirements, 
% one type of agents at a time.
% A problem arises is that
% updated agents with new policies may not be able to cooperate with 
% other types of old agents with old policies, and vice versa.
% Although we can update the policy of all types of agents easily in simulations,
% in reality it can cost a lot to stop machine agents in production.

% Therefore, a method to iterate policies without breaking the compatibility 
% between different heterogeneous agents
% is needed in order to actually apply the multiagent systems to application.


==> tex_bk/2-rel.tex <==
\section{Related Works}

Although Heterogeneous Multiagent Reinforcement Learning (HMARL) is not a new problem in MARL,
they have not yet been investigated extensively in the literature.
While there are works introducing model-based HMARL algorithms on specific domains, 
e.g., traffic control, medical information processing, and control system 
\cite{calvo2018heterogeneous, kishor2021reinforcement, fard2022time, chen2020off},
a general-purpose heterogeneous reinforcement learning is absent as far as we're concerned.
On one hand,
tasks stressing their heterogeneous property are likely to have solid application backgrounds and concerns on realistic problems.
On the other hand,
existing simulation and training frameworks cannot support flexible task customizations
for heterogeneous systems.

While most environments only consider homogeneous 
agent tasks \cite{baker2019emergent, deka2021natural, zheng2018magent, fu2022concentration},
benchmark environments that contain heterogeneous agent cooperation are also emerging.
Multi-Agent Particle Environment (MAPE) \cite{lowe2017multi}
is a simple but flexible multiagent environment,
design for less sophisticated tasks such as predator-prey and speaker-listener.
However, MAPE is a lightweight framework designed for 2D environments and lacks further extensibility.
The SMAC benchmark environment proposed in \cite{samvelyan2019starcraft}
provides some examples of heterogeneous team combinations such as 1c3s5z and MMM2,
however, as an RTS game based environment,
existing SMAC maps only support up to 27 agents (homogeneous map),
and only one of the maps (MMM2) considers the supporting relationship within
team agents.
Moreover, despite there being tools for making SMAC maps, 
SMAC still lacks customizations for building new agents, 
designing inter-team interaction or simulating realistic tasks.

Existing MARL studies address tend to address heterogeneous agent cooperation implicitly,
without specially distinguishing from homogeneous ones \cite{rashid2018qmix, rashid2020weighted}.
Firstly,
all agents are given the same action space despite their type,
except that some particular actions are invalid concerning some of the agent types.
secondly,
agents are not explicitly modeled according to their type,
instead, 
agents need to discover their abilities and strengths by interacting with the environment and teammates.
Such practice is successful in many tasks with weak agent ability distinction 
because agent experience can be shared regardless of agent type.
However, in complex heterogeneous problems, 
the agent policy cannot be generalized from one type to another,
meaning that agents cannot benefit from sharing their experiences with different-type agents.


In recent years, 
efficient algorithms based on multiagent systems are developed 
without explicit agent-type consideration.
In early models such as IQL (Independently Q-Learning) \cite{watkins1989learning},
each agent learns its own policy independently.
Then \cite{lowe2017multi} points out the non-stationary problem 
when directly migrating single-agent approaches to multiagent environments.
In \cite{lowe2017multi} a MADDPG algorithm is proposed 
for stabilizing multiagent RL 
based on DDPG (Deep Deterministic Policy Gradient \cite{lillicrap2015continuous}).
Moreover, \cite{sunehag2017value} proposed a Q-learning-based algorithm VDN,
and the model is further improved by Qmix \cite{rashid2018qmix}, and Weighted Qmix \cite{rashid2020weighted},
which use hyper-networks \cite{ha2016hypernetworks} to decompose the task reward signals.
Other algorithms \cite{foerster2018counterfactual, yang2020q}
provide further improvement by leveraging the counterfactual advantage function
and integrated gradient et.al.
Nevertheless,
classic MARL methods ignore the quantity difference between agent types,
which can cause non-stationary between heterogeneous agents and
has a negative impact on algorithm performance.

% when solving heterogeneous problems.
% due to the great difference between different types agents,
% the policy cannot be generalized from one type to another.


%

% because agents can usually share their experience across the 

% agents cannot observe whether another agent is of the same type,
% and learn










% % type A -> type B transfer
% Nevertheless, 
% due to the great difference between different types agents,
% the policy cannot be generalized from one type to another.

% % 加剧了Non-stationary问题
% % Unlike homogeneous multiagent tasks,
% The non-stationary issue is one of the difficulties
% presented by heterogeneous multiagent problems.
% In heterogeneous multiagent tasks,
% different kinds of agents var in ability, quantity,
% expected functionality etc.
% Notably the quantity of each agent type is unbalanced in most scenarios.
% E.g., in military simulations,
% high-value aircrafts are essential for obtaining battlefield advantage 
% but are very few in number compared with ground agents.
% This imparity is also common in the world of nature, 
% e.g., in a hive honey bees queens and workers differ greatly in number.

% The unbalanced number of agents leads to
% more inaccurate state value estimation for agents that are few in number,
% compared with other agents. % put forward theory, then start explaining
% In MARL agents learn from samples collected 
% via interacting with the environment.
% Unlike homogeneous multiagent tasks,
% agents belonging to different types cannot share their experience.
% For example, a patrol UAV cannot share its experience with
% a ground agent since they do not have the same ability and functionality,
% and they may even have different available action space.
% As a result,
% agents with numerious same-type companions
% are likely to learn faster and establish more precise
% estimation concerning their situation, 
% while agents with very few same-type partners (or no partners at all)
% develop their knowledge much more slowly.
% % As a consequence,
% % some agents will learn faster than others,
% This disordered and uncoordinated learning process 
% will further aggravate non-stationary of 
% agents perception towards environment,
% causing issues in MARL learning efficiency.

% % Heterogeneous多体问题是真实世界的映射，真实世界中的不稳定性问题
% As a saying goes, no two snowflakes are alike.
% There is no absolute homogeneous cooperation game in the world of nature.
% Also, considering cost and reliability, homogeneous robot system 
% is usually better than homogeneous systems in artificial systems.
% Studying the cooperation between heterogeneous agents
% bring us one step closer to applying reinforcement learning to
% real world applications.

% One of the gaps between reality and MARL theory is that
% the policy version iteration problem.
% In a heterogeneous systems,
% different types of machine agents are likely manufactured by
% different companies at different time.
% In reality, after put into use,
% we may still need to update the hardware of agents and then 
% train them to adapt the updated hardware according to new requirements, 
% one type of agents at a time.
% A problem arises is that
% updated agents with new policies may not be able to cooperate with 
% other types of old agents with old policies, and vice versa.
% Although we can update the policy of all types of agents easily in simulations,
% in reality it can cost a lot to stop machine agents in production.

% Therefore, a method to iterate policies without breaking the compatibility 
% between different heterogeneous agents
% is needed in order to actually apply the multiagent systems to application.


% \section{Heterogeneous MARL}
% A heterogeneous MARL task can be described as a Dec-POMDP \cite{oliehoek2016concise},
% which can be formulated by 
% $\langle A, \varDelta, \mathcal{U}, \mathcal{S}, P_t, \mathcal{Z}, P_o, r , \gamma\rangle$,
% where $A$ is the collection of agents and $N=|A|$ is the total number of agents.
% $\mathcal{U}$ is a collection of actions within which each agent $a_i$ can choose from.
% $\mathcal{S}$ is the set of environment states and $P_t$ is the transition function.
% $r$ is team reward. $\gamma$ is the discount factor.
% In a heterogeneous system, 
% $\varDelta = \lbrace \delta_1, \dots, \delta_{n_j} \rbrace$ is the set of agent types and 
% $n_j = |\varDelta|$ is the total number of types in the system.
% Each agent $a_i$ is categorized into a type $\text{Type}(a_i) = \delta_j$.
% Although the quantity of agents can be large,
% the the number of types is very limited $n_j \ll N$,
% since in the real world
% agents (usually robots) 
% are usually manufactured via standardized production to reduce cost.




% \section{Method}

% \subsection{League Training}
% League training is first introduced in AlphaStar \cite{vinyals2019grandmaster}.
% To effectively improve agents' initial capability,
% AlphaStar takes advantage of human expert data to train agents with a supervised approach,
% obtaining a population of agents with different policies.
% Agents are subsequently trained with reinforcement learning,
% and intermittently duplicate themselves and freeze these duplications as past players.
% The agent players are trained against each other as well as themselves in history.
% AlphaStar agent was rated at Grandmaster level in Starcraft game.

% % The significant advantage of league training is that 
% % it enables agent to learn adaptive policies which considers the different strategies of opponents.
% League training enables agents to learn adaptive and robust policies against 
% continually developping strategies of other fellow agents,
% which also has great value in heterogeneous MARL in order to 
% solve the policy iteration problem and to improve model performance.

% Unfortunately, league training cannot be applied to heterogeneous MARL because of following reasons.
% First and most importantly,
% heterogeneous agents collaborate instead of competing in heterogeneous MARL.
% (If there are two or more adversarial teams, a unit entity is refered to as an agent only in its own team).
% Secondly,
% there will be no human data for supervised pre-training.
% Thirdly,
% League training used by \cite{vinyals2019grandmaster} consumes huge amount of computational resource and 
% it will be too expensive to be applied elsewhere.

% \subsection{Heterogeneous League Training Framework}
% \subsubsection{League Collaborating Hyper Network}
% Cooperating with a variety of partners with different policies is challenging.
% Some partners are well-trained and willing to cooperate,
% while some partners using past policies frozen at not-trained states can only behave randomly.
% It is necessary to equip agents with a neural network structure 
% that is sensitive to the differences of heterogeneous partners.

% For a heterogeneous team with agents $\lbrace a_1, \dots, a_{N} \rbrace$,
% we use a tuple $\langle \alpha,  \rangle$
% \begin{equation}

% \end{equation}

% describe the 
% aware of
% A hyper-network structure to solve the conflicts of cooperating with 
% different versions of agent partners.



% To

% By making agent players competing with others and themselves in history,
% eventually overcome continually adapting strategies.


% which spawns a great population of player agents.
% we 

% Traditionally,
% when training a multiagent systems


% If we can find a way to iterate policies 
% without breaking the compatibility between different types of agents,

% To finish such updates a problem must be solved.

% it is    a hardware update or 

% it is common for human operators to spot flaws

% it may be inconvenient or impossible to replace

% different types of agents are manufectured by different

% One of the concern arise in homogeneous systems






% For example,
% many methods use attention mechanism to process large observation space,
% but different types of agents may have to learn distinct ways to
% pay attention diff

==> tex_bk/3-prelim.tex <==
\section{Preliminaries}
\subsection{Heterogeneous MARL.}
A heterogeneous MARL task can be described as a Dec-POMDP \cite{oliehoek2016concise},
which can be formulated by 
$\langle A, \varDelta, \mathcal{U}, \mathcal{S}, P_t, \mathcal{Z}, P_o, r , \gamma\rangle$,
where $A$ is the collection of agents and $N=|A|$ is the total number of agents.
$\mathcal{U}$ is a collection of actions within which each agent $a_i$ can choose from.
$\mathcal{S}$ is the set of environment states and $P_t$ is the transition function.
$r$ is the team reward. $\gamma$ is the discount factor.
In a heterogeneous system, 
$\varDelta = \lbrace \delta_1, \dots, \delta_{n_j} \rbrace$ is the set of agent types and 
$n_j = |\varDelta|$ is the total number of types in the system.
Each agent $a_i$ is categorized into a type $\text{Type}(a_i) = \delta_j$.
Although the quantity of agents $N$ can be large,
the the number of types $n_j$ is considerably smaller ($n_j \ll N$),
this is because in the real world agents (usually robots) 
are usually manufactured via standardized production to reduce cost.
Furthermore, considering the cost,
it is common that agents of high-value types are lesser in number 
than cheap agents in a functional heterogeneous team.

\subsection{League Training in AlphaStar.}
League training is first introduced in AlphaStar \cite{vinyals2019grandmaster}.
To effectively improve agents' initial capability,
AlphaStar takes advantage of human expert data to train agents with a supervised approach,
obtaining a population of agents with different policies.
Agents are subsequently trained with reinforcement learning,
and intermittently duplicate themselves and freeze these duplications as past players.
The agent players are trained against each other as well as themselves in history.
The trained AlphaStar agent was rated at Grandmaster level in the Starcraft II game.

% The significant advantage of league training is that 
% it enables agents to learn adaptive policies which consider the different strategies of opponents.
League training enables agents to learn adaptive and robust policies against 
continually developing strategies of other fellow agents,
which also has great value in heterogeneous MARL to 
solve the policy iteration problem and improve model performance.

Unfortunately, league training cannot be applied to heterogeneous MARL for the following reasons.
First and most importantly,
heterogeneous agents collaborate instead of competing in heterogeneous MARL.
(If there are two or more adversarial teams, a unit entity is referred to as an agent only in its own team).
Secondly,
there will be no human data for supervised pre-training.
Thirdly,
League training used by \cite{vinyals2019grandmaster} consumes a huge amount of computational resources and 
it will be too expensive to be applied elsewhere.



==> tex_bk/4-hlt.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%Heterogeneous League Training%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Heterogeneous League Training}

\begin{figure}[!t]
  \centering
  \includegraphics[width=\linewidth]{img/league-crop.pdf}
  \caption{Heterogeneous League Training framework.}
  \label{fig:main-fig}
  \end{figure}


Next, we propose a Heterogeneous League Training (HLT) algorithm motivated AlphaStar,
an efficient and general-purpose multiagent reinforcement learning algorithm for heterogeneous cooperative systems.

In this section, 
we start by stating our motivation and model features in Sec~\ref{sec:motivation}, 
e.g., our league training model is designed to promote the ability to cooperate instead of competing.
Next,
we briefly introduce the general framework of HLT in Sec~\ref{sec:framework}.
Then,
the details of heterogeneous league training is further presented in Sec~\ref{sec:LeagueSampler} and Sec~\ref{sec:LeagueManagement}.
Finally,
as an essential structure to achieve adaptive cooperative behaviors,
the design of hyper-networks is illustrated in Sec~\ref{sec:hyper}.



\subsection{Motivation and Features.}
\label{sec:motivation}
HLT aims at two goals in heterogeneous multiagent RL:
\begin{itemize}
  \item Taking advantage of the feature of heterogeneous systems to facilitate cooperation.
  \item Addressing the policy iteration problem.
\end{itemize}

\subsubsection{Motivation.} 

The following reasons inspired us to use the league training technique to achieve our goals.
Firstly, 
different agent types vary considerably in quantity.
Samples that the RL algorithm collected from episodes
can provide low-variance experiences for types with numerous agents (T+). On the other hand, 
types with comparably fewer agents (T-) receive high-variance experience.
The learning process becomes unstable when T- agents fail to catch up with the progress of T+ agents,
and T+ agents give up counting on T- agents and 
turn to develop uncooperative policies that exclude the help of T-.
By adopting the cooperative league training technique,
agents optimize their policies 
not only from the experience of cooperating with each other,
but also from the experience of teaming up with foreign agents with different cooperation skills. % (parameter-frozen) 
More specifically,
cooperative league training technique addresses the learning instability problem 
by encouraging agents to use different cooperation behaviors depending on who their teammates are.

Secondly,
cooperative league training provides an environment where
agents are trained to work with a league of heterogeneous teammates 
equipped with diverse collaboration preferences.
By adding history agent policies into the league,
agents can learn new cooperative behaviors 
while not forgetting the way to collaborate with old versions of heterogeneous teammates.


\subsubsection{Key Features.} 

First and most importantly,
AlphaStar is an example of a \textbf{adversarial} multiagent league training algorithm, 
where agents are trained to compete.
What we propose in this paper is a \textbf{cooperative} league training method, 
which is designed to facilitate heterogeneous agent cooperation.

Secondly,
AlphaStar league model requires distributed servers with TPUs to run concurrent matches,
but our algorithm only needs a single machine with a single GPU 
to execute the whole training process.
To achieve this, 
we redesign the procedure of the league training based on 
the characteristic of heterogeneous systems.
Furthermore,
we introduce a hyper-network structure, 
facilitating each agent with the ability to change its cooperative behavior 
according to its type and the performance of its heterogeneous teammates.




\begin{figure*}[!t]
  \centering
  \includegraphics[width=0.8\linewidth]{img/framework-crop.pdf}
  \caption{Policy optimization cycle.}
  \label{fig:optimization}
  \end{figure*}

\subsection{Overall Framework of HLT.}
\label{sec:framework}

\subsubsection{Actors and Critic.}
Our Heterogeneous League Training (HLT) model 
follows the Centralized-Training-Decentralized-Execution (CTDE) paradigm.
Agents learn the type identities of the whole heterogeneous team from the observation,
in which each agent's type is described by a one-hot vector.
Agents belonging to the same type share the policy network parameters,
while agents from different types can choose freely 
between using shared network parameters or using independent networks.
Therefore, 
we use a term \textbf{policy group} (denoted as $\vec{\pi}$) to describe the policy/policies
of an entire heterogeneous team.
For generality,
policies for each agent type are represented by:
$$
  \vec{\pi} = \lbrace \pi(\delta_1),\dots, \pi(\delta_M) \rbrace
$$
where $ \delta_1, \dots, \delta_{n_j} $ represent each agent type.
Note that each policy $\pi(\delta_j)$ controls all $\delta_j$ agents in the team.

The computational cost is a serious concern in cooperative multiagent systems.
Consequently, we only initialize and optimize one dynamic policy group during league training.
This policy group is referred to as the \textbf{frontier policy group} or $\vec{\pi}_{\text{f}}$.

We establish a policy pool referred to as a league $\mathcal{L}$ to hold history policies,
similar to AlphaStar.
As shown in Fig.\ref{fig:main-fig}, 
a series of past policies is intermittently duplicated and separated from the frontier, 
and then placed into the past pool during training.
Once independent from the frontier,
the network parameters of past policies are frozen
so that we only need to compute policy gradient for frontier policies 
instead of for all policies in the pool.
Those frozen policies in the league are referred to as \textbf{past policy groups}.
Let $|\mathcal{L}|$ be the total number of policies in the league,
each member policy group is denoted as:
$$\mathcal{L}=\lbrace 
\vec{\pi}_{\text{p},1}, \dots, \vec{\pi}_{\text{p},|\mathcal{L}|}
 \rbrace
$$


Additionally,
while there are different groups of policy networks (as actors) in HLT,
there is \textbf{only one critic network} in HLT to action assessment during the whole training process.

\subsubsection{Optimization Iteration.}
As illustrated in Fig.~\ref{fig:main-fig},
the algorithm begins with a randomly initialized policy group and an empty league.
This group of random policies is the initial frontier policy group.
When each policy optimization iteration is done,
the new policy group (frontier) will be evaluated by a filter,
determining whether it is distinct from the policies already inside the league.
If the new frontier deviates much from policies in the league,
it will be accepted as a new league member.
Otherwise, the league stays unchanged till the next iteration.

In each optimization iteration, 
if the league is empty,
agents directly interact with the environment with the frontier policy group,
and collect episode samples for initial policy optimization.
When the league contains past policy groups,
agents will randomly sample policies from both the frontier and the league
for policy optimization.

\begin{figure*}[!t]
  \centering
  \includegraphics[width=0.8\linewidth]{img/hypernet-crop.pdf}
  \caption{Hyper network for learning adaptive cooperative behavior.}
  \label{fig:hyper}
  \end{figure*}

\subsection{League Sampler.}
\label{sec:LeagueSampler}
\label{sec:x}

As shown in Fig.~\ref{fig:optimization},
the frontier policy group is trained to cooperate not only with itself,
but also with past policies that it visited previously during the learning process.

For each episode,
the league sampler randomly generate a policy combination $C_{\text{sel}}$.
This combination is either frontier-past
$C_{\text{sel}}=(\vec{\pi}_{f}, \vec{\pi}_{\text{p},l})$, 
or frontier-frontier
$C_{\text{sel}}=(\vec{\pi}_{f} , \vec{\pi}_{f})$.
The balance between frontier-frontier and frontier-past combination 
is adjusted by a constant hyper-parameter $p_f \in \left[0,1\right)$:
\begin{equation}
\begin{array}{ll}
  &P\left[C_{\text{sel}}=\left( \vec{\pi}_{f}, \vec{\pi}_{\text{p},l} \right)    \mid p_f \right] = \frac{1}{(1-p_f)|\mathcal{L}|} \\
  &P\left[C_{\text{sel}}=\left( \vec{\pi}_{f}, \vec{\pi}_{f}          \right)    \mid p_f \right] = p_f
\end{array}
\end{equation}
where $|\mathcal{L}|>0$ and $p_f<1$. 
When the league is empty ($|\mathcal{L}|=0$), 
league sampler provides only frontier-frontier combination, 
namely $C_{\text{sel}}=( \vec{\pi}_{f}, \vec{\pi}_{f} )$.
When $p_f=0$, the sampler avoids the pure frontier combination 
and always samples one of the past policy groups from the league in $C_{\text{sel}}$.
On the other hand,
when $p_f \approx 1$, 
the sampler tends to exclude the participant of the league.






Next, 
a combination sampler receives $C_{\text{sel}}$ and 
eventually determines the policy that each agent executes.
For clarity, we use $\vec{\pi}_\text{sel}$ and $C_{\text{sel}} = (\vec{\pi}_f, \vec{\pi}_\text{sel} )$ to represent 
the selected policy group and the combination respectively.
As shown in Fig.~\ref{fig:optimization}, 
the combination sampler choose one of the agent type to play the past policies, 
each type has an equal probability of being selected,  regardless of the number of agents it possesses:
$$
  P(\delta_j) = \frac{1}{|\varDelta|}, \forall \delta_j \in \varDelta
$$
Finally, with an agent type $\delta_t$ chosen to use the corresponding policy in group $\vec{\pi}_\text{sel}$.
The mix policy group $\vec{\pi}_{\text{mix}}$ that the team executes is:
$$
  \vec{\pi}_{\text{mix}} = \lbrace \pi_{\text{mix}}(\delta_1),\dots, \pi_{\text{mix}}(\delta_M) \rbrace
$$
where
$$
    \pi_{\text{mix}}(\delta_j) = \left\{\begin{array}{ll}
        \pi_f(\delta_j),            & \delta_j \neq  \delta_t \\
        \pi_{\text{sel}}(\delta_j), & \delta_j = \delta_t
    \end{array}\right., \forall \delta_j \in \varDelta
$$

The mix policy group $\vec{\pi}_{\text{mix}}$ only influences one episode.
But the league sampler and combination sampler can generate 
a batch of different $\vec{\pi}_{\text{mix}}$ to run in parallel.
This process is repeated to collect a batch of episodes for frontier policy optimization.
The policy gradient w.r.t. the frontier policy parameters is calculated from the collected episodes
and used to optimize each frontier policy of each agent type.


  
\subsection{League Member Management.}
\label{sec:LeagueManagement}
\label{sec:xx}
To be able to run on a single machine, HLT has to control the size of the league. 
In AlphaStar, researchers use a sizeable past agent pool which costs a significant amount of memory and time,
which is not applicable to most heterogeneous problems.
From the intuition that the league should contain policies with diverse behaviors and distinct cooperative abilities,
we use a league filter to manage and control the league size as shown in Fig.\ref{fig:optimization}.

In HLT, a metric $\Omega \in [0,1]$ is introduced to compare the similarity of policy groups.
This metric can be the success rate, normalized test reward 
(projecting the minimum reward and maximum reward to 0 and 1, respectively),
or any other evaluation scores that reflect policy performance.

Let $|\mathcal{L}|_{\text{max}}$ be the maximum size of the league.
if the size of the pool exceeds $|\mathcal{L}|_{\text{max}}$,
the league filter deals with policy group candidates using the following procedures:
\begin{itemize}
\item (1) evaluate the new policy group with metric $\Omega$.
\item (2) add the policy group into the league.
\item (3) sort all policy groups in the league according to their $\Omega$ metric.
\item (4) the league filter finds a pair of policy groups with the closest evaluation metric and then removes the newer group.
\end{itemize}


More specifically, since the league capacity is exceeded during step (2)\~(4):
$$\mathcal{L}=\lbrace \vec{\pi}_{\text{p},1}, \dots, \vec{\pi}_{\text{p},|\mathcal{L}|+1}  \rbrace$$
to find a policy group to remove, 
we first evaluate each past policy group with  metric $\Omega$:
$$
\Omega(\mathcal{L}) = \left\lbrace   \Omega(\vec{\pi}_{\text{p},1}), \dots,    \Omega(\vec{\pi}_{\text{p},|\mathcal{L}|+1})     \right\rbrace = \lbrace \omega_1, \dots, \omega_{|\mathcal{L}|_{\text{max}}+1} \rbrace
$$
where $\omega_1, \dots, \omega_N, \omega_{|\mathcal{L}|_{\text{max}}+1}$ are evaluation scores.
Then the league is sorted according to $\omega$ scores,
rearranging $\mathcal{L}$ so that:
$$
\omega_1 \le \dots \le \omega_N \le \omega_{|\mathcal{L}|_{\text{max}}+1}
$$
Finally, find a pair of policy groups $\vec{\pi}_{\text{p},k}$ and $\vec{\pi}_{\text{p},k+1}$ with closest evaluation metric:
$$
     |\omega_{k+1} - \omega_{k} | \le |\omega_{k'+1} - \omega_{k'} |, \quad \forall k' \in [1, |\mathcal{L}|_{\text{max}}]
$$

Then the order of when group $k$ and group $k+1$ are added into the pool is considered. We always remove the newer policy group within $\vec{\pi}_{\text{p},k}$ and $\vec{\pi}_{\text{p},k+1}$.
By removing the relatively newer group instead of the older one,
we can avoid frequent changes inside the league and prevent potential instability.
After removal, the size of the league reduces back to $|\mathcal{L}|_{\text{max}}$.

\subsection{Adaptive Hyper Network.}
\label{sec:hyper}
\label{sec:xxx}
% Cooperating with a variety of partners with different policies is challenging.
% Some partners are well-trained and willing to cooperate,
% while some partners using past policies frozen at not-trained states can only behave randomly.
% It is necessary to equip agents with a neural network structure 
% that is sensitive to the differences of heterogeneous partners.


Cooperating with a variety of partners with different policies is challenging.
Agents of any type may encounter strong heterogeneous partners that are well-trained and cooperative,
on the other hand,
they may also meet weak heterogeneous partners using past policies frozen at immature stages.
It is necessary to equip agents with a neural network structure 
that is sensitive to the differences of heterogeneous partners.
In HLT, 
we use a hyper-network structure to achieve this goal.

As shown in Fig.~\ref{fig:hyper}, 
the hyper-network is a structure to generate network parameters for MLP layers in the main policy network.
Internally, 
the hyper-network uses two layers of fully connected networks to produce MLP parameters,
using an agent-team information vector $F_h$ as input.

The agent-team information vector $F_h$ is determined by agent type $\delta_j$ and the mixed policy $\vec{\pi}_{\text{mix}}$. 
It is a concatenation of two parts:
$$
F_h(\delta_j, \vec{\pi}_{\text{mix}}) = \operatorname{concat}\left[ \ 
    F_{v}(\delta_j, \vec{\pi}_{\text{mix}}) 
    , \ 
    F_{\delta}(\delta_j) \  
    \right]
$$
$F_{\delta}$ is a one-hot binary vector for distinguishing agent types. 
E.g, if $\delta_j=\delta_1$, then $F_{\delta}(\delta_j)=F_{\delta}(\delta_1)=[1, 0, 0, \dots]$.
And $F_{v}(\delta_j, \vec{\pi}_{\text{mix}})$ represents the combination of the mixed heterogeneous team 
by identifying the policy that each agent type executes. 
$$
    F_{v}(\delta_j, \vec{\pi}_{\text{mix}})  = (V_{\delta_1},\dots,V_{\delta_{|\varDelta|}})
$$

$$
    V_{\delta_j}=\left\{\begin{array}{ll}
            1,                                      & \delta_j \neq  \delta_\text{sel} \\
            \Omega[\pi_{\text{sel}}(\delta_j)],     & \delta_j = \delta_\text{sel}
    \end{array}\right., \quad \forall \delta_j \in \varDelta
$$
where $V_{\delta}$ describes frontier policies with constant $\Omega_\text{max}= 1$ and past policies with the metric $\Omega$ of their policy group.
Since $\Omega[\pi_{\text{sel}}(\delta)] < 1$ before the completion of training,
$V_{\delta}$ always illustrates the difference between frontier policies and past policies.

Specially,
we also need to consider the hyper-network input for past policies.
As mentioned previously,
all past policies are duplications of the frontier policy at a certain stage,
they, same as the frontier policy, were always trained under the circumstance 
where they observe themselves as the frontier, i.e., $V_{\delta} = 1$.
For consistency, 
past policies still observe themselves as frontiers with $V_{\delta}=1$.
Concretely,
differing from $F_h$,
past policies use $\hat{F}_h$ as hyper-network input:
$$
\hat{F}_h(\delta_j, \vec{\pi}_{\text{mix}}) = \operatorname{concat}\left[ \ 
    [1,1,\dots,1]
    , \ 
    F_{\delta}(\delta_j) \  
    \right]
$$

Afterward, the hyper-network produces a vector of parameters $\theta_h$:
$$
\theta_h = \text{HyperNet}(\hat{F}_{v})
$$
Two MLP layers are used as the structure of the hyper-network.
The vector $\theta_h$ is split and reshaped 
into weight matrix $w_h$ and bias vector $b_h$,
which work as feed-forward layers $f$ in the main policy network:
$$
    f( h | \theta_h) = \text{Relu} (w_h h + b_h)
$$
where $h$ represents the input of the network layers.



% For a heterogeneous team with agents $\lbrace a_1, \dots, a_{N} \rbrace$,
% we use a tuple $\langle \alpha,  \rangle$
% \begin{equation}

% \end{equation}

% describe the 
% aware of
% A hyper-network structure to solve the conflicts of cooperating with 
% different versions of agent partners.


==> tex_bk/5-exp.tex <==
\section{Experiments}


\begin{figure}[!t]
  \centering
  \includegraphics[width=0.6\linewidth]{img/uhmp-f1-crop.pdf}
  \caption{A map of Unreal-based Hybrid Multiagent Platform (UHMP), 
  with 2 support UAVs and 8 ground agents on each side.}
  \label{fig:uhmp-f1}
  \end{figure}

\begin{figure}[!t]
  \centering
  \includegraphics[width=0.5\linewidth]{img/uhmp-f3-crop.pdf}
  \caption{ An illustration of supportive UAV agents.
  Supportive UAV agents (Type 1) are responsible for repairing and assisting nearby agents, 
  equipped with missile-weapon payload but are vulnerable to opponent attacks.
  }
  \label{fig:uhmp-f3}
  \end{figure}
      

\begin{figure}[!t]
  \centering
  \includegraphics[width=0.5\linewidth]{img/uhmp-f2-crop.pdf}
  \caption{An illustration of two types of ground agents. 
  Agents of the second type (Type 2) are ground units with missile-weapon payload.
  Agents of the third type (Type 3)  are ground units with kinetic-weapon payload.
  }
  \label{fig:uhmp-f2}
  \end{figure}


  
\subsection{Heterogeneous Benchmark Environment.}
The heterogeneous league training algorithm is tested under
the Unreal-based Hybrid Multiagent Platform (UHMP),
an advanced heterogeneous simulation environment.
As shown in Fig.\ref{fig:uhmp-f1} and Fig.\ref{fig:uhmp-f3},
we use a built-in AI as the opponent of the HMARL learner,
two teams share symmetrical configurations.
Moreover, 
we use tags such as \text{2u-4m-4k} and \text{2u-4m-14k} to represent the configurations.
E.g.,
the sequence \text{2u-4m-4k} indicates the type and number of heterogeneous agents in each team.
Each team has 2 supportive air-borne UAV agents ($\delta_1$, \text{2u}), 
capable of attacking, 
repairing allies and reducing damage caused by opponents.
The other 8 agents are ground units.
Half of them have missile-weapon payload and long attack range ($\delta_2$, \text{4m}).
Other ground units ($\delta_3$, \text{4k}) equip kinetic weapons with short attack ranges
and are incapable of attacking opponent UAVs.
$\varDelta = \lbrace \delta_1, \delta_2, \delta_3 \rbrace$ and $|\varDelta| = 3$.

The functionality of different agents in UHMP is also shown in Fig.\ref{fig:uhmp-f2} and Fig.\ref{fig:uhmp-f2}.
Due to the ability difference,
agents belonging to one type have to learn policies 
that are, to an extent, unshareable to other heterogeneous types.
Furthermore,
due to the imparity of quantity between different types,
the importance and learning difficulty of agent types diverges from one another.


\subsection{Algorithm Performance Evaluation.}
\subsection{Experimental Setup.}

We run our experiments on a single Linux server with regular AMD CPUs and Nvidia GPUs (RTX 8000),
and we only use one GPU for each experiment.
PPO and Adam optimizer are used for applying policy gradient on policies neural networks.
We adopted dual-clip PPO and policy resonance techniques to improve training efficiency.
To control the league's involvement,
we set $p_f=0.1$ for the league sampler by default
so that in 90\% of all episodes,
agents execute mixed policies with the participant of both frontier and past policies.
We set $|\mathcal{L}|_\text{max} = 5$ because running a large number of past policy groups concurrently 
can significantly slow down the model calculation.
We frequently evaluate the frontier policy group with the winning rate as the metric $\Omega$,
and we average the results of 160 episodes in every evaluation for precision,
the intermittent evaluation takes place once every 1600 training episodes.
In experiments, we run each experiment setting repeatedly with at least four different random seeds.


\subsection{Performance of HLT.}
To test the effectiveness of the proposed HLT model,
we compare the proposed HLT method with existing SOTAs 
such as FT-Qmix (fine-tuned Qmix) \cite{hu2021rethinking}.

While individual observations alone suffice the requirements of HLT,
some of those methods (such as Qmix) require an extra state information vector 
during centralized training.
Determining how the additional states are obtained,
we use the '-D' suffix to represent a model trained 
in a Delicately designed state space,
or no suffix to represent a model trained 
in an untuned state space (or not using state information at all).



% We investigate how
% We examine whether both chosen motivational indices are essential.
% (a) We assess how the concentration parameter dc influences the module. 
% (b) We investigate whether the extra
% self-attention layer shown in Fig. 1 provides improvement.
% (c) We examine whether reducing our model from DualConcNet to Single-ConcNet causes a performance decay.
% (d) We investigate whether Conc-4Hist model can utilize
% history observations under extreme interference.

\subsection{The Effectiveness Against Policy Iteration Problem.}
\label{PolicyIteration}
We investigate how the HLT model improves the policies compatibility 
between different versions of policies.
When the training is completed,
we test whether a fully trained policy group (the eventual frontier policy group) 
can promote the win rate of past policies when mixed together.
In this test,
we still use the random combination sampler introduced previously 
for the following tests of frontier-past policy compatibility:
\begin{itemize}
  \item For each episode, randomly select one type of agent that executes the past policies 
    while the types of agents execute the frontier policies. (Frontier exclusive test.)
  \item For each episode, Randomly select one type of agent that executes the frontier policies, 
    while the types of agents execute the past policies. (Frontier inclusive test.)
  \end{itemize}


In the former test, 
the frontier policy group controls most types of agents.
With the frontier policy group being the majority in the team, 
we assess how the frontier works with the minority of agents 
controlled by past policies with various cooperation capabilities.
In the latter test,
we examine how the frontier policies respond to a scenario where
most agents are using past policies.
Playing a minority type in a heterogeneous team without a dominant position,
this challenges the frontier's capability to adapt.

\subsection{Investigation on Heterogeneous Role Learning.}
In the policy iteration test, 
we sample the type combination randomly and 
only focus on the frontier's adaptive ability as a group.
However,
it is also valuable to investigate the difference 
between frontier policies (which control different types of agents).
This experiment provides us with a way to assess the difficulty of 
learning each heterogeneous role,
and furthermore offer a new perspective for
analyzing how a cooperative heterogeneous 
the joint policy comes into existence.



\section{Results.}

\subsection{Main Results.}
We compared our HLT method with other SOTAs on two main common metrics, 
namely win rate and test reward.
Each score is averaged over 160 test episodes, 
and then averaged again over 
at least four independent experiments launched by different random seeds.

\begin{table}[!t]
  \centering
  \setlength{\tabcolsep}{0.5mm}{
    \begin{tabular}{ccc}
      \toprule
      {Algorithm} 
                                      & {Best Test Win Rate}  
                                                              & {Best Test Reward}         \\
      \midrule
      {HLT         }  
                                      & \textbf{98.09\%}              
                                                              & \textbf{1.782}      \\
      {FineTuned Qmix} 
                                      & {87.98\%}              
                                                              & {1.452}   \\
      {FineTuned Qmix-D}              
                                      & {91.79\%}              
                                                              & {1.547}   \\
      \bottomrule
  \end{tabular}
  }
  \caption{
    Performance comparison between methods.
  }
  \label{table:performance}
\end{table}
From the results shown in Fig.\ref{table:performance},
HLT has the best performance among all models 
despite that HLT does not use any state information.
FineTuned Qmix also has a relatively good performance 
when trained by a delicately designed global state.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Heterogeneous Cooperation Policy.}

Observing the finalized policies trained by HLT,
we find a clear agent role division between different agent types.
Fig.\ref{fig:uhmp} demonstrates a scenario where 
green RL agents are preparing to contact the enemy.
T1 agents (UAVs) take advantage of their agility 
by moving back and forth 
to attack enemies and simultaneously support ground teammates.
T2 agents have a longer attack range than T3,
but they learned a hit-and-run policy,
moving ahead of T3 agents when opponents are far but 
immediately retreat behind T3 agents when facing threats.
The strength of T3 agents is short-range combat,
but being in a heterogeneous team, they learn
a rather sedate policy, 
which stays still when the simulation begins
and then forms a circle formation along with T2 when opponents approach.





\begin{figure*}[!t]
  \centering
  \begin{subfigure}[t]{0.32\linewidth}
  \centering
  \includegraphics[width=\linewidth,height=0.6\linewidth]{uhmp/s1.jpg}
  \caption{Step 4. T2 advancing.}
  \label{fig:dca1}
\end{subfigure}
%  
\begin{subfigure}[t]{0.32\linewidth}
  \centering
  \includegraphics[width=\linewidth,height=0.6\linewidth]{uhmp/s2.jpg}
  \caption{Step 8. T3 advancing.}
  \label{fig:dca2}
\end{subfigure}
%  
\begin{subfigure}[t]{0.32\linewidth}
  \centering
  \includegraphics[width=\linewidth,height=0.6\linewidth]{uhmp/s3.jpg}
  \caption{Step 11. Circle formation.}
  \label{fig:dca3}
\end{subfigure}
%  
\caption{Cooperating with clear role division. HMARL algorithm controls the green team, 
and the opponents are represented in blue color.
The moving direction of agents is represented by circles and red arrows nearby each agent in figures.}
\label{fig:uhmp}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Policy Compatibility.}

Fig.\ref{fig:win_rate_absolute_improvement_both}
demonstrates the win rate improvement when
the frontier policy group interferes with the past policy groups.
The past policy groups have different levels of cooperative ability,
quantified by their $\Omega$ metric (independent win rate).
We use past policy groups with $\Omega < 0.90$,
which are more distinguishable from the frontier policy group with $\Omega \approx 1$.
We use two kinds of the test described in Sec~\ref{PolicyIteration},
frontier exclusive test results are represented by blue samples,
and frontier-inclusive test results are shown with red samples.
A significant improvement can be observed in the policy group 
with $\Omega \in (0.2, 0.6)$ in both tests,
the participants of the eventual frontier policy promote 
the win rate notably above the green $\Omega$ baseline,
this suggests an affinity can be established between the frontier and those past policies.
When $\Omega > 0.7$, 
the room for improvement is very limited,
but in most experiments, frontier policies can still provide compatibility for those policies 
without raising conflicts that ruin the cooperation win rate.



\begin{figure}[h]
  \centering
  \includegraphics[width=0.6\linewidth]{img/win_rate_absolute_improvement_both_addicon.pdf}
  \caption{Compatibility between finalized policies and past policies. 
  Win rate with the participant of eventual frontier policies.}
  \label{fig:win_rate_absolute_improvement_both}
\end{figure}


% \begin{figure}[h]
%   \centering
%   \includegraphics[width=0.6\linewidth]{img/win_rate_improvement_both.pdf}
%   \caption{Compatibility between finalized policies and past policies. 
%   Improvement with the participant of eventual frontier policies.
%   }
%   \label{fig:PolicyIteration}
% \end{figure}


% \begin{figure}[h]
%   \centering
%   \includegraphics[width=0.6\linewidth]{img/win_rate_improvement_both.pdf}
%   \caption{A wrong images.}
%   \label{fig:win_rate_improvement_both}
% \end{figure}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Heterogeneous Role Learning.}
\begin{figure}[h]
  \centering
  \includegraphics[width=0.6\linewidth]{img/ReplaceTest1_addIcon_final.pdf}
  \caption{Revealing heterogeneous role learning process 
  by mixing the frontier and the past policies. (Frontier exclusive.)}
  \label{fig:ReplaceTest1}
\end{figure}

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=0.6\linewidth]{img/ReplaceTest2.pdf}
%   \caption{Revealing heterogeneous role learning process 
%   by mixing the frontier and the past policies. (Frontier inclusive.)}
%   \label{fig:ReplaceTest2}
% \end{figure}

All types of agents are essential in a heterogeneous task.
However,
the fact that different roles that agents learn vary in difficulty.
With the HLT model,
we can investigate and track the learning process of individual agent types.

The role learning process can be evaluated from two different aspects.
Fig.\ref{fig:ReplaceTest1} reveals the win rate decline 
when one of the agent types turns to execute past policies 
instead of the eventual frontier policy.
When $\Omega \approx 0$,
the past policies back then are almost random.
At this point, 
replacing the policy of T1 (UAVs) 
causes the most serious consequences (reducing win rate by 90\% on average),
while the influence of replacing the policy of T2 is relatively smaller.
This suggests that well-functioning T1 agents 
are most indispensable in the frontier policies compared with the other two agent types.
Nevertheless, T1 agents catch up fast with other agents 
when the policy group reaches $\Omega \approx 0.4$.
On the other hand,
T3 agents have the slowest win rate ascent among all three agent types,
and frequently becomes the black sheep after team $\Omega > 0.4$.
This indicates that the policy of T3 is usually the most difficult policy to learn.
However,
we also point out that the role-learning process is sophisticated,
the conclusion on the indispensability and learning difficulty of agent types 
is only based on statistics and may not stand in individual cases.
E.g., some individual experiment samples are outliers,
indicating a different situation 
is encountered in those particular training processes. 

% we also noticed that this result has a high variance in Fig.\ref{fig:ReplaceTest1},
% in some individual experiments,
% we 

% This does not suggests the difficulty of roles.


















% HLT和其他方法的胜率对比

% HLT和不使用HLT前后，策略兼容性对比

% HLT策略兼容性的进一步研究，定量化地展示每一个类别智能体对任务的重要性


==> tex_bk/6-conclusion.tex <==


\section{Conclusions}
In this work, 
we propose a Heterogeneous League Training (HLT) algorithm,
a general-purpose MARL algorithm for heterogeneous multiagent problems.
HLT introduces a light-weight league containing diverse agent policies 
gathered at different stages during training,
promoting the robustness of agent policies by training agents
with heterogeneous teammates with different cooperation skills.

Our results in cooperative heterogeneous tasks show that 
HLT improves the final performance compared with other existing methods.
And the policy compatibility experiments show that 
policies trained by HTL
can work together with immature past policies and promote their win rate.
Moreover,
HLT can statistically evaluate the difficulty of learning 
different roles in a heterogeneous team,
making it easier to identify the weakness of the heterogeneous cooperative system.






